Selfish & Opaque Transaction Ordering in the Bitcoin Blockchain: The Case for Chain Neutrality

Most public blockchain protocols, including the popular Bitcoin and Ethereum blockchains, do not formally specify the order in which miners should select transactions from the pool of pending (or uncommitted) transactions for inclusion in the blockchain. Over the years, informal conventions or "norms" for transaction ordering have, however, emerged via the use of shared software by miners, e.g., the GetBlockTemplate (GBT) mining protocol in Bitcoin Core. Today, a widely held view is that Bitcoin miners prioritize transactions based on their offered "transaction fee-per-byte." Bitcoin users are, consequently, encouraged to increase the fees to accelerate the commitment of their transactions, particularly during periods of congestion. In this paper, we audit the Bitcoin blockchain and present statistically significant evidence of mining pools deviating from the norms to accelerate the commitment of transactions for which they have (i) a selfish or vested interest, or (ii) received dark-fee payments via opaque (non-public) side-channels. As blockchains are increasingly being used as a record-keeping substrate for a variety of decentralized (financial technology) systems, our findings call for an urgent discussion on defining neutrality norms that miners must adhere to when ordering transactions in the chains. Finally, we make our data sets and scripts publicly available.

==> Makefile <==
MAIN=paper
SRCS=sections/*.tex

LMK=latexmk
OTYPE=-pdf
TEX=-pdflatex
TEX_OPTS="pdflatex -interaction=nonstopmode -shell-escape"
BIB=-bibtex

ERROR_MSG=Error: cannot find '$(LMK)' in path; try 'pdflatex $(MAIN).tex'

lmk_check =								\
	@which $(LMK) > /dev/null ||		\
		(echo "$(ERROR_MSG)" >& 2 &&	\
			exit 1)

default: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(SRCS)
	$(call lmk_check)
	@$(LMK) $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

.PHONY: watch clean

# Automatically rebuild latex files whenever changes are made.
watch: $(MAIN).tex
	$(call lmk_check)
	@$(LMK) -pvc $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

clean:
	@rm -f *.dvi *.aux *.blg *.log *.ps *~ *.bbl *.fdb_latexmk *.fls $(MAIN).pdf *.out


==> sections/diffobs.tex <==
\section{On differential observability}\label{sec:diff-obs}

In estimating the baseline blocks, we relied \stress{only} on the transactions
in our full-node's \mpool. This ``view'' of the \mpool, however, could be
substantially different from that of another node or miner simply because of
where that miner is geographically located.
Information on transactions introduced or blocks mined in the network
disseminates through the peer-to-peer network via a gossip protocol at different speeds depending, at
least, on the latency between the nodes in the network.
The discrepancies observed, $B_i \setminus \hat{B_i}$ and $\hat{B_i} \setminus B_i$, could,
perhaps, be explained by such network delays.
The \stress{ignored} transactions\footnote{Ignored by the miner and, hence,
missing in the actual block, but included in the baseline.} in $\hat{B_i} \setminus
B_i$, for instance, could have been committed in block $B_{i+1}$ or later
instead of $B_i$, perhaps because the miner received them later than when we
observed it.
They could also have been committed earlier in block $B_{i-1}$ or earlier
instead of $B_i$, perhaps because our full node observed these transactions
later than when the miner observed them.
We explore, hence, different scenarios that could explain the discrepancies and
ascertain whether to give miners the benefit of doubt---rather than flag their
behavior as a violation of the norm---and to what extent.


\begin{figure}[tb]
  \centering
  \begin{subfigure}[b]{\onecolgrid}
    \includegraphics[width={\textwidth}]{images/inter-block/top_5_txs_intersection_dist}
    \figcap{}
    \label{fig:ab-bb-common-top5-scatter}
  \end{subfigure}
  \begin{subfigure}[b]{\onecolgrid}
    \includegraphics[width={\textwidth}]{images/inter-block/txs_ignored_cdf}
    \figcap{}
    \label{fig:bb-ab-at-diff-time-thresh}
  \end{subfigure}
  \figcap{(a) All mining pools occasionally deviate from the norm. (b) Even with
    a 2-block cutoff period, miners ignore some transactions half the time}
\end{figure}

\subsection{Where ``our view'' is at fault}\label{subsec:our-view-lacking}

Let us suppose that the discrepancies between the baseline ($\hat{B_i}$) and
actual blocks ($B_i$) are due to our full node ``missing'' some of the
transactions observed by the miners. We now examine to what extent this premise
holds true.

\parai{Were miners privy to certain transactions?}
Of the set of transactions in $B_i \setminus \hat{B_i}$, we measured the fraction that
our full node \stress{never} observed in its \mpool.
In nearly $80\%$ of the $\num{3079}$ blocks, the full node does not miss even one
transaction; stated differently, transactions in $B_i \setminus \hat{B_i}$ were
observed, in most cases, at some point in time in our \mpool (and were included
in some baseline block, but not $\hat{B_i}$).
Even in the $99$-th percentile, the full node fails to observe fewer than $10\%$
of the transactions in $B_i \setminus \hat{B_i}$. These small number of cases could be
explained by network delays, resulting in some transactions being received after
``their'' blocks: Transactions received after the block, in which they were
included, causes the full node to drop the transaction (silently) even before
adding them to the \mpool.
\stress{Even if miners were being privy to certain transactions, the small
fraction of transactions our full node ``misses'' to observe cannot explain the
large discrepancies.}


\parai{Did we miss transactions with high fees?}
Recall that in computing the baselines we used the fee-per-byte metric to
prioritize transactions. If our full node missed some transactions with higher
fee-per-byte values than the minimum across all transactions in a given
baseline, these missed transactions will explain some of the discrepancies.
Across the $\num{3079}$ blocks in our data set, we observe, however, only $1\%$ of the
transactions in $\hat{B_i} \setminus B_i$ (i.e., observed in the baseline but not in the
actual) to have higher fee-per-byte values than the minimum across all
transactions in $B_i$.
\stress{Therefore, of the $22\%$ discrepancy (i.e.,
$\scriptstyle\frac{|\hat{B_i} \setminus B_i|}{|B_i|}$) we observe, only $1\%$ are
perhaps because of our full node missing some transactions with high fee rates.}

% \TODO{Provide some statistics on the fee-per-byte of these $1\%$ to further
% characterize the discrepancy. What does the distribution of the fee-rates of the
% 1\% look like?}

In summary, the transactions that our full node either never observes or fails
to observe ``on time'' explain, at best, a percent of those ignored (or absent)
in $B_i \cap \hat{B_i}$.


\subsection{Where ``their view'' is at fault}\label{subsec:their-view-lacking}

We are now left with only one premise to verify: Perhaps it is the miners who do
not observe some of the transactions ``on time''.

The ``All'' line in Figure~\ref{fig:bb-ab-at-diff-time-thresh} shows, for each
block, the number of (ignored) transactions in baseline but not in the actual block
(i.e., $\hat{B_i} \setminus B_i$) as a fraction of that in the actual block. For this
line to be true, every node in the peer-to-peer network should have observed the
transactions at the same time (i.e., with zero delays), which is infeasible.
To account for delays, we remove from this set of ignored transactions, those we
received within some \stress{cutoff period}, e.g., one minute, before a given
block is mined.
More concretely, if a transaction $t_i$ belongs to $\hat{B_i} \setminus B_i$, but the
time at which we received this transaction was within the cutoff period before
we received the actual block $B_i$, we drop it from the ignored set.
Per Figure~\ref{fig:bb-ab-at-diff-time-thresh}, the ``1 min.'' line, corresponding
to a $1$-minute cutoff period, significantly reduces the fraction of ignored
transactions: Fraction of ignored transactions drops (from $22\%$ in ``All'') to
$12\%$ or less; $2\%$ of the blocks (compared with \stress{none} in ``All'')
also have no ignored transactions.
Increasing the cutoff period to $2$ minutes further reduces the discrepancies,
in favor of the miners.

The cutoff period accounts for the scenario that perhaps the miners received the
transactions ``later'' than our full node.
It is unlikely, however, that the mining pools would experience a delay, as high
as, one minute: It is in the best interests (economically speaking) of the
mining-pools to equip their infrastructure with low-latency network connections,
after having spent millions in hardware~\cite{Zhao-WebArticle2019}; the fixed
infrastructure costs alone should reduce the cost of providing low-latency
Internet connectivity (e.g., \cite{FIBRE-URL2019} and \cite{Basu-Talk2016}) to
their nodes.
The economic argument notwithstanding, even with a 2-minute cutoff period,
$50\%$ of the blocks ignore nearly $10\%$ of the transactions.

Rather than use absolute time spans for the cutoff period we also used
block-based cutoff periods.
A one-block cutoff period implies that we drop any transaction in the ignored
set if it was received anytime before the current block $B_i$ (where it is being
flagged as ignored) but after we received the prior block $B_{i-1}$. Recall that
block generation times, in Bitcoin, vary with an average of about $10$ minutes.
Even with a two-block cutoff period (i.e., $20$ minutes on average), we observe,
in Figure~\ref{fig:bb-ab-at-diff-time-thresh}, $50\%$ of the blocks to have at
least some ignored transactions!

\stress{The analyses using (absolute) time-based as well as block-based cutoff
periods indicate that a significant fraction of transactions is being ignored
from immediate inclusion, for whatever reason, by miners.}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

==> sections/discussion.tex <==
\paraib{Potential explanations for broader norm deviations.}

% Our analyses, in Sections \S\ref{sec:mempool} and \S\ref{sec:interblock}, show
% that miners significantly deviate from what is widely believed to be the
% ``norm''---the same dequeuing policy as the \gbt mining protocol.
% More specifically, our analyses reveal that $22\%$ of the transactions per block
% do not seem to follow the rank ordering based on the fee-per-byte metric.
We now present a few conjectures, backed by empirical observations, that could
explain the miners' behavior.
%and its implications for the Bitcoin---or more
%generally the blockchain---ecosystem.


%\subsection{Musings on miners' behavior}
For each transaction, regardless of whether it was present in both the baseline
and actual blocks ($B_i \cap \hat{B_i}$) or only in the actual ($B_i \setminus \hat{B_i}$)
or just in the baseline ($\hat{B_i} \setminus B_i$), we compute the transaction delay as
the difference between when the transaction was received in \mpool and when it
was included in the baseline or actual, depending on to which of the three
aforementioned categories the transaction belongs.
Figure~\ref{fig:tx-delay-diff-class} shows the CDF of the delays for all
transactions, separately for each of the three categories.

\begin{figure}[tpb]
  \centering
  \begin{subfigure}[b]{\onecolgrid}
    \includegraphics[width={\textwidth}]{images/inter-block/txs_delay_cdf.pdf}
    \figcap{}
    \label{fig:tx-delay-diff-class}
  \end{subfigure}
  \begin{subfigure}[b]{\onecolgrid}
    \includegraphics[width={\textwidth}]{images/inter-block/txs_feerate_cdf.pdf}
    \figcap{}
    \label{fig:tx-feerate-diff-class}
  \end{subfigure}
  \figcap{(a) It is unlikely that the miners are ignoring transactions because
    these arrived too close to when the block was mined: Some, if not all, of
    the transactions in $B_i \setminus \hat{B_i}$ arrived minutes later than those in
    $B_i \cap \hat{B_i}$. (b) Transactions in $B_i \setminus \hat{B_i}$ have significantly
    lower fee-per-byte compared to those in $B_i \cap \hat{B_i}$, suggesting that
    fee-per-byte does not completely explain miners' dequeuing policies.}
\end{figure}

Per Figure~\ref{fig:tx-delay-diff-class}, some of the transactions that the miners
included (in the actual block) that are not in the baseline (i.e., the category
$B_i \setminus \hat{B_i}$) arrived several minutes later than those that appear in both
the actual and baseline blocks (i.e., the category $B_i \cap \hat{B_i}$).
Some of the transactions in the baseline but not in the actual block (i.e.,
category $\hat{B_i} \setminus B_i$), arrived much earlier compared to those in the $B_i
\setminus \hat{B_i}$.
\stress{Perhaps the miners are using a different protocol, which takes other parameters,
in addition to fee-per-byte, into consideration.}


\stress{Perhaps the miners are being ``altruistic''.}
Said differently, miners might be committing transactions that have been waiting
in the \mpool for a ``long'' time, despite those transactions having
comparatively lower fees---the CDF of $|B_i \setminus \hat{B_i}|$ in
Figure~\ref{fig:tx-delay-diff-class} lends some credence to this line of
reasoning.
Figure~\ref{fig:tx-feerate-diff-class}, which is similar to
Figure~\ref{fig:tx-delay-diff-class} except that the x-axis is transaction fee
rate instead of delays, also shows that the transactions prioritized by
miners have comparatively lower fee rates.
The observation that $60\%$ or more of the transactions that have been waiting
for 10 minutes or longer (in the CDF of $|\hat{B_i} \setminus B_i|$ in
Figure~\ref{fig:tx-delay-diff-class}) were ignored by the miners, however, clearly
refutes the claim of an ``altruistic'' behavior.

\stress{Are miners adopting other strategies?}
We hypothesize that mining pool operators might be sending a different set of transactions to each miner (or perhaps changing this set every a fixed time interval or event) to reduce the network overhead, avoiding miners to request a new task often. It is possible due to the stratum protocol\footnote{Stratum is a pooled mining protocol available at \url{https://stratumprotocol.org}}. Stratum is a pooled mining protocol that focuses on reducing network communication between the mining pool and its miners by allowing miners to change some bytes on the coinbase transaction and consequently changing the Merkle root. Another reason is that some clients might be using services like transaction accelerators to speed up the commit time of a particular transaction. They pay the mining pool to use this service off-chain (i.e., with another cryptocurrency or via credit-cards) to, hopefully, increase the probability of their transactions get included in the next block. One example of this service is the \textit{BTC.com transaction accelerator}\footnote{\textit{BTC.com} is one of the biggest Bitcoin mining pools operators currently available. Its transaction accelerator service is available at: \url{https://pushtx.btc.com/}}.


\paraib{Implications.}
%
Regardless of whether the miners are altruistic,
Figure~\ref{fig:tx-feerate-diff-class} strongly suggests that the dequeuing policy
is not simply a function of the fee-per-byte metric.
The transactions in $B_i \setminus \hat{B_i}$ have, for instance, significantly smaller
fees than those available in $B_i \cap \hat{B_i}$. Further, the $B_i \cap \hat{B_i}$
and $B_i \setminus \hat{B_i}$ lines in Figure~\ref{fig:tx-feerate-diff-class} suggest that
even if users pay a fee significantly higher---one or two orders of magnitude
higher---than the lowest fee ($\uTxFee{e-5}$), there is virtually no guarantee
that their transaction will be included in the next block.
Only beyond an exorbitant fee rate ($\uTxFee{e-1}$) there is, unsurprisingly, a
guarantee that the concerned transaction will be immediately committed.
Today, virtually all of the fee predictors, however, falsely assume that miners
follow the fee-per-byte metric for prioritizing transactions for inclusion.



\if 0
\section{Discussion}\label{sec:discussion}

\subsection{Impact of non-transparent }

\subsubsection{On the right norm(s) for transaction prioritisation:}

\subsubsection{Enforcing the right norm:}

\subsubsection{Fairness of }
\fi

% \begin{figure}[htb]
%   \includegraphics[width={\onecolgrid}]{images/inter-block/txs_ignored_congested_non_congested_cdf}
%   \caption{}
%   \label{fig:cumsum-empty-blocks}
% \end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> sections/interblock.tex <==
\section{On Transaction Commit Prioritization}\label{sec:interblock}


In a decentralized system, it is vital that all participants follow a ``norm,''
to avoid compromising the stability and fairness of the system.
%
Bitcoin Core~\cite{BitcoinCore-2019}, the widely used software to access the
Bitcoin blockchain history, uses the fee-per-byte metric (or the \GBT
protocol~\cite{GBT-Bitcoin-2019}), for prioritizing transactions for inclusion.
%
Miners, hence, should use \GBT as the ``norm.''
%
In this section, we check the adherence of miners to this norm.



\subsection{Broader deviations from the norm} \label{subsec:deviations-from-the-norm}

\if 0

% We showed in~\S\ref{subsec:feerates} that users respond to congestion by
% increasing transaction feerates.
% But how do users predict the feerates?
Having shown selfish violations of the norm for vested interest transactions, we now focus on norm violations for all transactions, in general.
If miners do not follow the norm for most transactions, feerate prediction has serious economic implications for the users. It could become even worse in the following years.
To justify our concerns of the miners' behaviors, we checked for transaction
pairs that unequivocally show that miners are not completely following the norm.
To this end we sampled, uniformly at random, $30$ \mpool snapshots
(see~\S\ref{subsec:cong-delays}) from the set of all available snapshots.
Suppose that, in each snapshot, we denote, for any transaction $i$, the time at
which it was received in the \mpool by $t_i$, its feerate by $f_i$, and the
block in which it was committed by $b_i$.
We then selected, from each snapshot, all pairs of transactions $(i,j)$ such
that $t_{i} < t_{j}$ and $f_{i} > f_{j}$, but $b_{i} > b_{j}$.
Each pair essentially has one transaction that appeared earlier and has a higher
feerate than the other, but still was committed later than the other; such pairs
clearly constitute a violation of the ``norm".

Bitcoin supports notions of dependent transactions, involving a parent and
child, where the child pays a high fee to incentivize miners to also confirm the
parent from which it draws its inputs. This mechanism enables users to
``accelerate'' a transaction that has been ``stuck'' because of low
fee~\cite{CoinStaker-2018}. As the existence of such \newterm{child-pays-for-parent (CPFP)} transactions 
would introduce false positives in our analysis we decided to discard them. 
Figure~\ref{fig:violation-non-cpfp}		
 shows that violations exist even after discarding all such dependent pairs.
Figure~\ref{fig:violation} shows a CDF of the percentage of the number of such
transaction pairs (line labelled ``$\ast$'') violating the norm across all sampled
snapshots.
Even if relax the time constraint as $t_{i} + \epsilon < t_{j}$ and use an $\epsilon$ of
either $10$ seconds or $10$~minutes, there exist (in Figure~\ref{fig:violation}) a
non-trivial number of violations.

\fi 

\paraib{Establishing a baseline.}


To systematically evaluate how well the fee-per-byte metric explains the
dequeuing behavior of miners, we establish a \term{baseline} as follows.
We run a full node and stamp each transaction added to the Mempool with the
\stress{chain length}. Chain length represents the number of blocks already
present in the blockchain when a given transaction was received in the node's
Mempool.
For every block $B_i$ mined (in reality, in Bitcoin), we estimate the
\stress{candidate} set of transactions that were available to the miner. More
concretely, the candidate set of $B_i$ comprises all transactions that were
observed in the Mempool before block $B_i$ but have not been confirmed yet.
We order the transactions within a candidate set using the fee-per-byte metric
(the same adopted on the \GBT mining protocol and well believed to be the norm) 
and create a \stress{baseline} block $\hat{B_i}$ of
the same size as that of $B_i$, i.e., $|B_i| = |\hat{B_i}|$, from the candidate set.
% \REVISIT{The use of the \GBT protocol for establishing baselines assumes that
% all nodes run Bitcoin core, and indeed publicly available statistics on the
% software run by the nodes confirm indicate that nearly $97\%$ of them use
% Bitcoin Core\footnote{Available at: \url{https://coin.dance/nodes}}}.
% To test this assumption, we looked at the \stress{inventory} (\inv) messages
% exchanged between the full node and its peers. \inv messages are used to share
% the inventories of objects (e.g., transactions and blocks) known to a
% node with other peers.
% If the receiver, after comparing against its own inventory, realizes that it
% does not have the object, it can send a follow-up request to the concerned peer
% to receive that object.
To simplify the analyses, we removed child-pays-for-parent transactions prior to
creating the baseline block.
The number of such transactions dropped out from both the baselines and actual
blocks, represents (in the median) $29.6\%$ of the size of the candidate sets.
% We defer the discussion of the effect of ignoring these transactions until after
% we present the evaluations using the baseline.



\paraib{Deviations from the baseline.}


We examined the blocks and transactions in data set \dsa and estimated the
baselines for $\num{3079}$ actual blocks, observed during this period.
The ratio of the size of the intersection between each actual block ($B_i$) and
its corresponding baseline ($\hat{B_i}$), i.e., $|{B_i}\cap\hat{B_i}|$, to the size
of the corresponding $B_i$ (or $\hat{B_i}$) quantifies the extent to which
miners adhere to the fee-per-byte dequeuing policy;
Figure~\ref{fig:ab-bb-common-all} plots the CDF of the ratios across all $\num{3079}$
blocks.
In the median, there is a $78\%$ overlap between actual and baseline blocks: The
fee-per-byte metric seems, on average, to explain the dequeuing of transactions
from the \mpool.

\if 0
\begin{figure}[tb]
   \centering
   \begin{subfigure}[b]{\onecolgrid}
     \includegraphics[width={\textwidth}]{images/violation/tx-violation-all.pdf}
     \figcap{All transactions}		
     \label{fig:violation-all}		
   \end{subfigure}		
   \begin{subfigure}[b]{\onecolgrid}		
     \includegraphics[width={\textwidth}]{images/violation/tx-violation-non_cpfp.pdf}		
     \figcap{Only Non-CPFP transactions}		
     \label{fig:violation-non-cpfp}		
   \end{subfigure}		
   \figcap{There exists a non-trivial fraction of transaction pairs across all		
     snapshots, clearly indicating that miners do not adhere to the norm.}
   \label{fig:violation}
 \end{figure}
\fi

The magnitude of the intersection between the baselines and actual blocks is,
however, not $100\%$!
$22\%$ of the transactions in the baselines do not appear in the corresponding
actual blocks, i.e., $B_i \setminus \hat{B_i}$; by symmetry, $22\%$ of the actual blocks
do not intersect with the corresponding baselines, i.e., $\hat{B_i} \setminus B_i$.
Succinctly, $22\%$ of the composition of a block on average deviates from the
``norm.''
There exist, hence, a significant number of transactions whose inclusion (or the
lack thereof) in corresponding actual blocks cannot be explained by the \GBT
like strategy where miners rank transactions based on a fee-per-byte metric.


\stress{Could the deviating behavior be attributed to a small subset of miners?}
Performing the same analysis (of quantifying the overlap between baseline and
actual blocks), but only for the blocks mined by the top five\footnote{Based on
the number of blocks mined by each pool over the three-week study period.}
mining pools (Figure~\ref{fig:ab-bb-common-top5-scatter}) indicates that the pools
exhibit almost identical behavior.
% A closer inspection of the fraction of overlaps, in
% Figure~\ref{fig:ab-bb-common-top5-scatter}, reveals that, of the five mining-pool
% operators, AntPool contributes to the most egregious deviations (i.e., fraction
% of overlap is less than $0.2\%$).
The CDFs in Figure~\ref{fig:ab-bb-common-top5} are similar to those for the bottom
five mining pools as well. The
discrepancies between actual and baseline blocks is consistent across all
miners, regardless of size: Deviations from the ``norm'' are consistent across
all mining pools (or miners).

\begin{figure}[tb]
  \center
  \begin{subfigure}[b]{\onecolgrid}
    \includegraphics[width={\textwidth}]{images/inter-block/txs_intersection_cdf.pdf}
    \figcap{}
    \label{fig:ab-bb-common-all}
  \end{subfigure}
  \begin{subfigure}[b]{\onecolgrid}
    \includegraphics[width={\textwidth}]{images/inter-block/top_5_txs_intersection_cdf}
    \figcap{}
    \label{fig:ab-bb-common-top5}
  \end{subfigure}
  \figcap{(a) In the median, $78\%$ of the transactions in baselines appear in
    the corresponding actual blocks, and (b) the observations are consistent
    across the top-5 mining-pool operators.}
    \label{fig:interblock}
\end{figure}

% This (uniform) lack of adherence to the \GBT protocol across the different
% mining pools has serious implications for the use of the fee-per-byte metric to
% determine transaction fees (or waiting times).

%\stress{Impact of congestion.}
%The CDF of the fraction of overlap between actual and baseline, computed for
%only the blocks observed during periods of congestion, ``Congested'' line in
%Figure~\ref{fig:ab-bb-common-all}, indicates that the deviations from the ``norm''
%(or \GBT) becomes more pronounced when there is \mpool congestion.
%In performing this analysis, we conservatively assume a block received at time
%$t$ to have experienced congestion, if the \mpool size during $10$-minute window
%prior to its arrival (i.e., in each one minute snapshot, as in
%Figure~\ref{fig:mempool-congestion}) \REVISIT{was consistently higher than $\uMB{1}$}.
%Also, deviations from the norm during off-peak times (``Non-congested'' line in
%Figure~\ref{fig:ab-bb-common-all}) are significantly lower than that during
%congestion.

%\TODO{Include a CDF plot describing the congestion and non-congestion analysis here.}


%% --- --- ---

% For every new valid transaction that is inserted into our nodes' MemPool it will also contain in its transaction data structure the current number of blocks already inserted into the Blockchain (which we call initial block height -- based on our nodes local view). This information is useful to determine which are the transactions available during the mining process of the next block (height+1) when the current number of blocks is height.

% Therefore, to have all transactions available for a given block height we proceed as follows:
% \begin{enumerate}
%     \item Given a block height (``h"), select only transactions with the initial block height lower than ``h". This step will give us all transactions that our node received before the respective block height ``h".
%     \item Now given the transactions set in step (1) we have to certify that there is no transaction which was previously inserted into the Blockchain before the analyzed block height "h". Therefore, we need to filter out all transactions which were inserted into the blockchain before the block height ``h". 
% \end{enumerate}

% Note: Possible limitation, we are not considering starved transactions (those transactions that were not inserted at some point into the Blockchain) 

% Now, for a given block height we could infer which were the transactions available for inclusion.

% Please keep in mind, our methodology, therefore, relies on the following assumptions:
% \begin{enumerate}
%     \item Filter out transactions which depend on other transactions.
%     \item Filter out their ancestors
%     \item In order to rebuild a block by selecting which transactions should be included first, we have selected the same number of transactions what was in the block mined by miners. This is necessary due to the transactions with its ancestors we had to remove from our data. 
% \end{enumerate}

% For a total of 3,119 blocks, we analyzed 3,081 (98.78\%) blocks as 38 (1.22\%) were empty.

% Figure \ref{fig:mempool-tx-intersection} shows the cumulative distribution function of the fraction of intersection between the transactions in the block we should expect (our block) and the block inserted into the Blockchain. On average, 75.3\% of the transactions appeared in both blocks. We also computed the standard deviation (10.61\%), minimum (0\%), 25-perc (72.12\%), median (78.1\%), 75-perc (81.7\%), and finally the maximum (98.41\%). Figure \ref{fig:mempool-top-5-tx-intersection} shows the results considering only the top-5 mining pool operators. Also, we show the distribution of the fraction of intersection per block height (see Figure \ref{fig:mempool-tx-intersection-dist} for all mining pool operators and Figure \ref{fig:mempool-top-5-tx-intersection-dist} for the top 5).

% Further, we aim to analyze the fraction of transaction that should be included in the block height ``h" but it was included in the next blocks which we call delayed transactions. Based on our analysis and methodology, we found that on average 9.44\% of the transactions were delayed and inserted into some block ahead. We also computed the standard deviation (11.23\%), minimum (0\%), 25-perc (3.15\%), median (5.86\%), 75-perc (10.88\%), and the maximum (100\%) fraction of delayed transactions in a block (see Figure \ref{fig:mempool-tx-postponed} and Figure \ref{fig:mempool-top-5-tx-postponed}). Similarly, we also plotted the distribution per block height and for the top 5 mining pool operators (see Figure \ref{fig:mempool-tx-postponed-dist} and Figure \ref{fig:mempool-top-5-tx-postponed-dist}).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:

